Turbocharging Gaussian Process Inference with Approximate Sketch-and-Project

Gaussian processes (GPs) play an essential role in biostatistics, scientific machine learning, and Bayesian optimization for their ability to provide probabilistic predictions and model uncertainty. However, GP inference struggles to scale to large datasets (which are common in modern applications), since it requires the solution of a linear system whose size scales quadratically with the number of samples in the dataset. We propose an approximate, distributed, accelerated sketch-and-project algorithm ($\texttt{ADASAP}$) for solving these linear systems, which improves scalability. We use the theory of determinantal point processes to show that the posterior mean induced by sketch-and-project rapidly converges to the true posterior mean. In particular, this yields the first efficient, condition number-free algorithm for estimating the posterior mean along the top spectral basis functions, showing that our approach is principled for GP inference. $\texttt{ADASAP}$ outperforms state-of-the-art solvers based on conjugate gradient and coordinate descent across several benchmark datasets and a large-scale Bayesian optimization task. Moreover, $\texttt{ADASAP}$ scales to a dataset with $> 3 \cdot 10^8$ samples, a feat which has not been accomplished in the literature.

==> sections/main/theory.tex <==
\section{Theory}
\begin{itemize}
    \item Show that distributing over machines improves the convergence rate (basically, put the time for a matvec into the convergence rate)
    \item Give a rate of convergence to the true posterior within a particular subspace---this should yield an improvement over the result in \citet{lin2023sampling}
\end{itemize}
\subsection{Fast convergence along top-$k$ subspace for GP inference}
% Let $\{(x_i,y_i)\}_{i=1}^{n}$ be the training data. 
% The posterior Gaussian process is characterized by $\mathcal{N}(m_{*|n}, K_{*,*|n})$, where we have
% \begin{align*}
%     & m_{*|n} = K_{*,n}(K + \lambda I)^{-1} y,\\
%     & K_{*|n}(x,x') = K(x,x') - K(x,X)(K + \lambda^2 I)^{-1} K(X, x).
% \end{align*}
% Note that the above inference task requires solving the linear system $(K_{n,n} + \sigma^2 I) \iterw{}{} = y$ for the posterior mean, and $(K_{n,n} + \sigma^2 I) \iterw{}{} = K_{n,*}$ for the posterior covariance. 
% In this section we provide a convergence guarantee along the top $k$-dimensional subspace of the covariance matrix $K_{n,n}$ using a tail-averaged scheme. 
% Let $\lambda = \sigma^2$ and denote $K + \sigma^2 I$ by $K_{\lambda}$ and let $Q_k$ denote an orthogonal projection on the top $k$-dimensional subspace of $K$. 
% Let $\lambda_i's$ denote the eigenvalues of $K$ in descending order.
% In this section, we provide a convergence guarantee for solving
As we have seen, being able to solve linear systems with $K + \lambda I$ efficiently is essential to GP inference via pathwise conditioning. 
Thus, our solver should possess strong convergence guarantees. 
Prior work \citep{lin2023sampling} has shown that the components of the solution most relevant for learning lie along the dominant eigenvectors of $K + \lambda I$.
In this section, we show that our proposed algorithm enjoys fast convergence along the dominant eigenspace of $K + \lambda I$ 
In particular, we show \znote{Add alg name later} converges initially at a fast condition-number free $\bigO(1/t)$-rate, before transitioning to an exponentially fast convergence rate that depends upon the conditioning of $K + \lambda I$.
\znote{Revise when Sections 2 and 3 are more fleshed out}


In our work, for theoretical results, we rely on drawing the subsampling matrices from Determinantal Point Processes ($\dpp$). 
These subsampling matrices satisfy strong guarantees; such as providing an exact characterization of the expected projection matrix that arises in the analysis of \sapfull{}.
We use the following known result for fixed size $\dpp$s:

\begin{lemma}[Expected projection under $\hdpp{2s}(A)$, adapted from Lemma 4.1 \citep{dy24}]\label{lemma:fix_size_dpp}
Let $A \in \R^{n\times n}$ be a symmetric positive definite matrix and let $1 \leq s < n/2$ be fixed. 
Let $S \sim \hdpp{2s}(A)$. 
Then
\begin{align*}
\E[A^{1/2} S^T (S A S^T)^\dagger S A^{1/2}] = V D' V^T,
\end{align*}
where $D'$ is a diagonal matrix with $j^{th}$ diagonal entry lower bounded by $\frac{\lambda_j}{\lambda_j +\frac{1}{s}\sum_{i>s}{\lambda_i}}$.
\end{lemma}

Furthermore, approximate sampling from fixed-size $\dpp$s of positive-definite matrices can be done efficiently, as shown in the following result.

\begin{lemma}[Sampling from $\hdpp{2s}(A)$, adapted from \citep{dy24,anari2024optimal}]\label{lemma:dpp_sampling}
Given a positive-semidefinite matrix $A$, there exists an algorithm that draws $t \geq 1$ approximate samples from $\hdpp{2s}(A)$ in time $O(n s^2 \log^4 n + t  s^3 \log^3 n)$. 
Furthermore, each drawn sample is indistinguishable from an exact sample from $\hdpp{2s}(A)$ with probability at least $1-n^{-O(1)}$.
\todo{probably needs to be rephrased}
\end{lemma}

Now consider solving the linear system $K_\lambda x = y$ using \sapfull{}. 
The update rule is

\begin{align}
&\iterw{t + 1}{} = \iterw{t}{} - S^T (S K_\lambda S^T)^{-1} S (K_\lambda w_t - y) \nonumber \\
  \text{or equivalently}  \ K_\lambda^{1/2}(& w_{t+1} - \wstar) = (I - \projS) K_\lambda^{1/2}(\iterw{t}{} - \wstar), \label{eqn:rcd_update}
\end{align}
where $\projS = K_\lambda^{1/2} S^T (S K_\lambda S^T)^{\dagger} S K_\lambda^{1/2}$. 
The following is the main result of this section:

\begin{theorem}[Subspace convergence for GP inference]\label{theorem:fast_convg_gp}
Let $s < n/2$ be fixed and $S \in \R^{2s \times n}$ be a random subsampling matrix sampled from $\hdpp{2s}(K_\lambda)$.
Furthermore, let $1 \leq k < s$ be also fixed and $\lambda_k(\eproj) \geq 2 \lambda_n(\projS)$. 
For any $t > 1$ define $\bar w_t = \frac{1}{t} \sum_{i=t}^{2t-1} \iterw{i}{}$ where all $\iterw{i}{}$ are generated using the \sapfull{} update (\ref{eqn:rcd_update}). 
Then
  \begin{align*}
     \E\|K_\lambda^{1/2} (\bar w_{t} - \wstar)\|_{Q_k}^2 & \leq \left( 1 - \frac{s}{s + \sum_{i>s}{\frac{\lambda_i + \lambda}{\lambda_k + \lambda}}} \right)^t \|K_\lambda^{1/2} \wstar \|_{Q_k}^2 \\
     & + \frac{4}{t} \left( \frac{1}{s}\sum_{i>s}{\frac{\lambda_i+\lambda}{\lambda_k+\lambda}} \right) \left( 1-\frac{s}{n \bar \kappa_s(K_\lambda)} \right)^t \|K_\lambda^{1/2} \wstar \|^2,
     \end{align*}
     where $\bar\kappa_s(K_\lambda) = \frac{1}{n-s}\sum_{i>s}{\frac{\lambda_i+\lambda}{\lambda_n+\lambda}}$. 
\end{theorem}

\begin{corollary}[Subspace convergence for posterior mean]\label{corollary:fast_convg_gp}
Let $\wstar = K_\lambda^{-1} y$ and $\epsilon > 0$ be fixed. 
Furthermore, assume that $\lambda_i's$ decay at least polynomially i.e., $\lambda_i =\bigO(i^{-1})$. 
Then, with probability at least $0.9$,
\begin{align*}
     \E \| K_\lambda^{1/2} (\bar w_t -\wstar) \|_{Q_k}^2 & \leq \epsilon \| K_\lambda^{1/2} \wstar \|^2_{Q_k}
     \end{align*}
for $s = \bigO(k \log n)$ and $t=\bigO\left(\frac{n}{k} \min\{\frac{1}{\epsilon}, \bar\kappa_s(K_\lambda)\}\log(\frac{n}{\epsilon})\right)$. 
The total time complexity is $\bigO \left(n k^2 \log^6 n + (n^2 + nk^2 \log^5 n) \min \{\frac{1}{\epsilon}, \bar \kappa_s(K_\lambda) \} \log(\frac{n}{\epsilon}) \right)$.
\end{corollary}

\pnote{Let's hide log factors in $\bigOt$}

\pnote{Why does the theorem not depend on $w_0$?}

\pnote{Why does the RHS in the theorem contain $\|K_\lambda^{1/2} w^\star \|^2$?}

\mnote{Below is a possible way to present our results (needs to be double checked).}

\begin{theorem}
    Let $K$ and $y$ represent $n$ observations from a GP prior with variance $\lambda>0$. Also, let $\mathrm{proj}_k$ denote the orthogonal projection onto the subspace of the top $k$ eigenvectors of $K$, and let $r_k = k + \sum_{i>k}\frac{\lambda_i(K)}{\lambda_k(K)}$ denote the $k$-effective rank of $K$. Then, in time $\tilde O(nr_k^2)$ we can construct a subsampling distribution $S\in\R^{O(r_k)\times n}$ such that sketch-and-project initialized at zero obtains:
    \begin{align*}
        \E\,\big\|\mathrm{proj}_k(\bar x_t) - \mathrm{proj}_k(x^*)\big\|_{K_\lambda}^2
        \leq \frac Ct \bigg(1 - c\min\Big\{\frac {r_k}n,\frac \lambda{\lambda_k(K)}\Big\}\bigg)^t\|y\|_{K_\lambda^{-1}}^2,\quad\text{where}\quad\bar x_t = \frac 2t\sum_{i=t/2}^t x_i.
    \end{align*}
    Thus, we can find $\hat x$ that satisfies $\|\mathrm{proj}_k(\hat x) - \mathrm{proj}_k(x^*)\|_{ K_\lambda}^2\leq \epsilon\cdot \|\mathrm{proj}_k(x^*)\|_{K_\lambda}^2$ with prob. $0.99$ in
    \begin{align*}
    \tilde O\bigg( (n^2 + nk^2)\min\Big\{\frac1\epsilon, \Big(1 + \frac{r_k\lambda_k}{n\lambda}\Big)\log(1/\epsilon)\Big\}\bigg)\quad\text{time}.
    \end{align*}
\end{theorem}
\begin{remark}
    If the matrix $K$ exhibits polynomial spectral decay, i.e., $\lambda_i(K) =\Theta(i^{-\beta})$ for $\beta>1$, then for any $k\in\{1,...,n\}$, the $k$-effective rank satisfies $r_k=O(k)$.
\end{remark}

\mnote{Some comments:
\begin{itemize}
    \item  This puts less emphasis on DPP sampling. We could still discuss the sampling after the main theorem, but that way, it is less jarring that it doesn't appear later.
    \item On the right hand side of the convergence bound, $\|y\|_{K_\lambda^{-1}}^2$ can be replaced by $\|x^*\|_{K_\lambda}^2$, which is also with high probability bounded by $O(n/k)\|\mathrm{proj}_k(x^*)\|_{K_\lambda}^2$.
    \item We should be able to express the error in terms of the posterior mean $m$,  something like $\|\mathrm{proj}_k(\hat m) - \mathrm{proj}_k(m)\| \leq \epsilon \cdot\|\mathrm{proj}_k(m)\|$, but not sure what norm we should use.
    \item Note that this achieves $O(1/t)$ rate in terms of the \emph{squared} norms. If we take a square root on both sides, then we recover the $O(1/\sqrt t)$ rate of Lin et al. However, we still get a condition number free rate, which they do not.
\end{itemize}
}
